Bilateral Unsymmetrical Graph Contrastive Learning for Recommendation

Recent methods utilize graph contrastive Learning within graph-structured user-item interaction data for collaborative filtering and have demonstrated their efficacy in recommendation tasks. However, they ignore that the difference relation density of nodes between the user- and item-side causes the adaptability of graphs on bilateral nodes to be different after multi-hop graph interaction calculation, which limits existing models to achieve ideal results. To solve this issue, we propose a novel framework for recommendation tasks called Bilateral Unsymmetrical Graph Contrastive Learning (BusGCL) that consider the bilateral unsymmetry on user-item node relation density for sliced user and item graph reasoning better with bilateral slicing contrastive training. Especially, taking into account the aggregation ability of hypergraph-based graph convolutional network (GCN) in digging implicit similarities is more suitable for user nodes, embeddings generated from three different modules: hypergraph-based GCN, GCN and perturbed GCN, are sliced into two subviews by the user- and item-side respectively, and selectively combined into subview pairs bilaterally based on the characteristics of inter-node relation structure. Furthermore, to align the distribution of user and item embeddings after aggregation, a dispersing loss is leveraged to adjust the mutual distance between all embeddings for maintaining learning ability. Comprehensive experiments on two public datasets have proved the superiority of BusGCL in comparison to various recommendation methods. Other models can simply utilize our bilateral slicing contrastive learning to enhance recommending performance without incurring extra expenses.

==> ______.tex <==
mot图 坐标放大

-- 主图改改

切割模块的名字考量

method部分
四个小标题图上没有反映
4.4. 直接起名dispersing loss
-- 4.3.的小标题，在图上画个框突出重点，框起embs后标出来
4.3. 多写点理解，1和2点到为止
1+2合并将三个GCL  起名叫BusGCL结构  把章节名下面这一段/caption改换进去
4.5留着
【把‘图结构’和‘子图对比’分开】

-- 大图caption简写

尝试另外的GCN出来的emb的readout进行预测

check有没有切分sub-view的<推荐>文章，若有，写到relatedwork的C-part

relatedwork根据新的小标题来改

主实验结果的多个模型类别写到2.1

超参实验小标题 第一个直接写layer的

超参实验试一下 只对比一边的

超参尝试一个别的GCN替换Hyper/Perturb

消融实验找一个disp对位的loss尝试一下

4.5 lambda reg 过小，我们设置为零

先做：图2修改，check relatedwork

abstract后面不要太cue超图

-- 大表第二好的标下划线

-- 大表的caption写加粗和下划线的意义
ablation表的caption写消融实验的第一段（缩写）




问题：
表的caption的字体固定，使得在caption里面写bold/underline说明很难看
